Region Embedding with Intra and Inter-View Contrastive Learning

Unsupervised region representation learning aims to extract dense and effective features from unlabeled urban data. While some efforts have been made for solving this problem based on multiple views, existing methods are still insufficient in extracting representations in a view and/or incorporating representations from different views. Motivated by the success of contrastive learning for representation learning, we propose to leverage it for multi-view region representation learning and design a model called ReMVC (Region Embedding with Multi-View Contrastive Learning) by following two guidelines: i) comparing a region with others within each view for effective representation extraction and ii) comparing a region with itself across different views for cross-view information sharing. We design the intra-view contrastive learning module which helps to learn distinguished region embeddings and the inter-view contrastive learning module which serves as a soft co-regularizer to constrain the embedding parameters and transfer knowledge across multi-views. We exploit the learned region embeddings in two downstream tasks named land usage clustering and region popularity prediction. Extensive experiments demonstrate that our model achieves impressive improvements compared with seven state-of-the-art baseline methods, and the margins are over 30% in the land usage clustering task.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> inputs/rebuttal.tex <==
\newpage
\setcounter{table}{0} 

% Thanks for your careful and valuable comments. We will explain your concerns point by points. 
\vspace{-0.3cm}
\section{Response to Reviewer 2}
%\textcolor{blue}{Q1: The authors claimed that when the adjacent matrix changes, graph-based region embedding methods incur high computational costs. The reviewer disagrees with that claim. The number of regions in a city is not very large. As a result, the adjacent matrix's dimension isn't too high, and the computational cost is affordable.}

% \noindent\textcolor{blue}{Q1: The computation cost of region adjacent matrix is affordable rather than too high.}
% \noindent\textcolor{blue}{Q1: Computational cost of adjacent matrices.}

\noindent\textcolor{blue}{\textbf{Computational cost of adjacent matrices.}}
% A1: 
We 
% agree with your comments and 
will withdraw the claim that constructing adjacent matrices has high computational costs in the future version. Yet we note that the adjacent matrices are defined based on heuristic-based measures in existing studies and not learnable. 
% still suffers from the heuristic measures, leading to potential information loss and achieving sub-optimal solutions because it lacks optimization.

%\textcolor{blue}{Q2: In this paper, a simple concatenation operation is used to fuse two-view embeddings. There is a lack of a well-designed fusion model to fuse these two-view embeddings.}

% \noindent\textcolor{blue}{Q2: There is a lack of a well-designed fusion model to fuse two-view embeddings instead of simple concatenation.}

\noindent\textcolor{blue}{\noindent\textbf{Fusion model.}}
%
% A2: Thanks for your valuable comments. 
% We conduct an additional ablation study on the fusion operations as follows. 
We consider those commonly used fusion operations, including average fusion, max fusion, gated fusion, neural networks (NN) based fusion and bilinear fusion, for comparison. In the NN based fusion, we concatenate two-view embeddings firstly and use a MLP neural network to extract fused representations. We use the same embedding %dimensions
size for all fusion operations. 
The experiment results are shown in %Table \ref{tab:fusion}. 
the following table. Among the newly studied fusion operations, the max fusion performs better in the land usage clustering task while the NN based fusion performs better in the popularity prediction task. However, all these operations lead to entangled region representations.
% , which may bring noises for both views. 
Instead, the disentangled multi-view representation by simple concatenation (adopted in this paper) can achieve the best results and the inter-view contrastive learning serves to propagate information across views.
\begin{table}[h]
	\renewcommand\arraystretch{0.9}
	\centering
	\tiny
	%\vspace{-0.25cm}
	\vspace{-0.1cm}
	%\caption{Ablation Study for Fusion Operations.}
	\vspace{-0.25cm}
	\label{tab:fusion}
	\resizebox{1.0\linewidth}{!}{
		\begin{tabular}{ccccccc}
			\toprule
			\multirow{2}{*}{\textbf{Operations}} & \multicolumn{3}{c}{{\it Land Usage Clustering}} & \multicolumn{3}{c}{{\it Popularity Prediction}}  \\
			\cmidrule{2-7}
			& NMI & ARI & F-measure & MAE & RMSE & $R^2$  \\ \midrule
			Average & 0.756 & 0.449 & 0.458 & \underline{231.02} & 353.47 & 0.489  \\
			Max & \underline{0.759} & \underline{0.466} & \underline{0.471} & 238.06 & 365.77 & 0.455  \\
			Gated & 0.736 & 0.414 & 0.432 & 246.38 & 380.54 & 0.408 \\
		    NN Based & 0.560 & 0.154 & 0.182 & 236.12 & \underline{347.02} & \underline{0.508} \\
			Biliner & 0.721 & 0.388 & 0.407 & 231.83 & 360.54 & 0.468 \\
			\cmidrule{1-7}
			Concat & \textbf{0.762} & \textbf{0.474} & \textbf{0.488} & \textbf{189.92} & \textbf{296.26} & \textbf{0.643} \\ \bottomrule
	\end{tabular}}
	\vspace{-0.4cm}
\end{table}

% \textcolor{blue}{Q3: There is a lack of details about mobility view operations. For example, how to build the heatmaps from mobility data. It is better to clarify that.}

% \noindent\textcolor{blue}{Q3: There is a lack of details about mobility view operations. For example, how to build the heatmaps.}

% A3:
\noindent\textcolor{blue}{\textbf{Mobility view operations.}}
%
There are two important operations for mobility view, namely heatmap construction and heatmap augmentation. 
The heatmap construction operation (detailed in the Problem Formulation section) sets an element of the heatmap as the number of trips concerning the corresponding regions and time slice of the element.
% For the heatmap construction, we detail it in the Problem Formulation section. 
%(Mobility view) 
% and it is the statistic results of human trajectories. We calculate the ratio of travels between region pair at each time slot as the element of mobility heatmaps.
% For the heatmap augmentation, we detail it in the Intra-view Contrastive Learning section.
The heatmap augmentation operation (detailed in the Intra-view Contrastive Learning section) adds a Gaussian noise to each element in a mobility heatmap. 

% \noindent\textcolor{blue}{Q4: The technological innovations are still limited.}

\noindent\textcolor{blue}{\textbf{Technical innovations.}} 
Please refer to our justifications of innovation in our response to Reviewer 4.
\if 0
Our innovations are detailed as follows: 1) we propose a new self-supervised task to preserve the urban relation named intra-region \& inter-view relation (certain POI types corresponds to specific mobility patterns) which is not captured in  previous methods. 2) we propose a hierarchical contrastive learning framework in both intra-view and inter-view for the first time, which provides insights for further research. 3) we fill in the gap that combining contrastive learning with region representation and extensive experiments validate %our model's
its impressive performance.
\fi

% A4: 
%Our innovations can be detailed as follows: 1) we model a new relation named intra-region \& inter-view relation %(certain POI types corresponds to specific mobility patterns due to urban fact) 
%which is not captured explicitly in previous region methods.
%2) we introduce two guidelines and propose a two-stage contrastive learning framework in region embedding for the first time, which can provide insights for further research. 
%3) extensive experiments validate our model's impressive performance in solving real-world urban problems. 
% For example, The improvements are over 40\% in land usage clustering and over 19\% in region popularity prediction.




\vspace{-0.3cm}
\section{Response to Reviewer 3}
% \noindent\textcolor{blue}{Q5: suggest release codes for replication studies.}

\noindent\textcolor{blue}{\textbf{Code release.}}
% A5: 
%Thanks for your advice. 
We provided the codes in the supplementary files and will release the codes once the paper is accepted. 
%We will release the codes.

% \textcolor{blue}{Q6: in Fig. 2, the same color means that regions are in the same cluster; however, across Figure 2(a)-(e), is the use of color coding for indexing the cluster consistent? What is the criterion for color coding? Is it the cluster size, measure of continuity, or something else?}

% \noindent\textcolor{blue}{Q6: in Fig. 2,  What is the criterion for color coding? the use of color coding is not consistent.} 
% \noindent\textcolor{blue}{Q6: in Fig. 2, the use of color coding is not consistent.} 

% A6: 

\noindent\textcolor{blue}{\textbf{Colors of clusters.}}
% Thanks for your comments. 
We use different colors for different clusters randomly in Fig. 2. In a newer version, we shall use the cluster size as the index of colors for better consistency.
% We use the random index currently. Each cluster corresponds a random color in each Figure. We will follow your comments and use the cluster size as the criterion to reorganize the Figures for color consistence. 

\vspace{-0.3cm}
\section{Response to Reviewer 4}

% \noindent\textcolor{blue}{Q7: The novelty is limited.}

% A7: Thanks for your comments. Please refer to A4 to R2.

% \textcolor{blue}{The manuscript is overall well written. The main concern is the novelty and the choices of baselines. Multi-view embedding learning is not a new topic, and there are many off-the-shelf models we can exlpore in the POI scenario. In this regard, the choice of baselines should not be limited in the POI domain. For example, the paper 'Menghan Wang, Yujie Lin, Guli Lin, Keping Yang, Xiao-Ming Wu:
% M2GRL: A Multi-task Multi-view Graph Representation Learning Framework for Web-scale Recommender Systems. KDD 2020: 2349-2358' is very similar to the manuscript in technique choice. The authors should include a discussion or experimental comparison to verify the novelty of proposed model.}

%\noindent\textcolor{blue}{Q8: There are many off-the-shelf multi-view embedding learning models we can explore in the POI scenario. The choice of baselines should not be limited in the POI domain. Especially, a discussion or experimental comparison to M2GRL should be included. }

% \noindent\textcolor{blue}{Q8: There are many multi-view embedding learning models we can explore in the POI scenario. Especially, a discussion or experimental comparison to M2GRL should be included. }

% \vspace{-0.3cm}
\if 0
A8: In this respect, the most related works are multi-view embedding alignment methods (such as DCCAE, DistAE, Devise and M2GRL). Most of them often extract view-specific embeddings using reconstruction or supervised tasks and align them in the hidden space. Compared with them, our method designs a new contrastive learning task in view-specific embedding learning, which helps to learn distinguished representations. In the ablation study, we also replace the carefully designed contrastive learning task with the reconstruction task (named ReMVC-MSE) and we can observe the performance decrease. 

For M2GRL, the intra-view task is to reconstruct the graph structure, which is not a contrastive paradigm based on data augmentations either. In addition, pre-defining the region graphs is non-trivial, which may suffer from the drawbacks mentioned in the Introduction section (heuristic-based measures and not learnable). In fact, we can also observe the performance decrease from Table \ref{tab:m2grl}.
\fi

% Thanks for raising this comment. 
There is a rich literature of multi-view representation learning: most of the methods were designed for specific views of data (e.g., images, texts, speeches, graphs, etc.) yet very few is generally applicable across different views of data. These methods can be roughly categorized as \emph{representation alignment methods} and \emph{representation fusion methods}: the former learn multi-view representations jointly with the alignment among different views used as regularizers/constraints and the latter learn representations of individual views separately and then fuse the representations as those for the multi-views. Below we justify the innovation and baseline choices of this paper.

\noindent\textcolor{blue}{\textbf{Innovation.}} Our method is a representation alignment method and differs from existing methods in: (1) it uses contrastive learning to learn representations within a view (i.e., intra-view representation learning); and/or (2) it uses contrastive learning to regularize the representations across views (i.e., inter-view representation learning); and/or (3) it is tailored for region data with POI view and mobility view. In fact, we are aware of no existing methods which use hierarchical contrastive learning for both intra-view and inter-view representations learning as ours does.

In the M2GRL paper, which is mentioned by the reviewer, each view corresponds graph data and the intra-view presentation learning is based on reconstruction. That is, compared with M2GRL, our method differs in (1) and (3).

\noindent\textcolor{blue}{\textbf{Baseline choices.}} We compared with all methods that have been proposed for region representation learning based on POI and mobility views, including MV-PN, GCAL, and MVURE (results are in Table 2 of the paper). Among them, MV-PN and GCAL are more like representation alignment methods and MVURE is a representation fusion method, thus covering both categories of multi-view representation learning methods. We also compared with ReMVC-MSE, which replaces the intra-view contrastive learning of our method ReMVC with reconstruction-based representation learning, as an ablation study (results are in Table 3 of the paper and also %Table 2 of this response). 
the table below in this response). Finally, as suggested by the reviewer, we compared with M2GRL (results are in %Table 2 of this response). 
the following table). In summary, we have considered 5 baseline methods of multi-view representation learning methods, which we believe well represent the state-of-the-art methods for multi-view region presentation learning on region data. 

\vspace{-0.25cm}

\begin{table}[h]
	\renewcommand\arraystretch{0.9}
	\centering
	\tiny
	%\caption{Comparision with M2GRL.}
	%\vspace{-0.25cm}
	\vspace{-0.1cm}
	\label{tab:m2grl}
	\resizebox{1.0\linewidth}{!}{
		\begin{tabular}{ccccccc}
			\toprule
			\multirow{2}{*}{\textbf{Methods}} & \multicolumn{3}{c}{{\it Land Usage Clustering}} & \multicolumn{3}{c}{{\it Popularity Prediction}}  \\
			\cmidrule{2-7}
			& NMI & ARI & F-measure & MAE & RMSE & $R^2$  \\ \midrule
			M2GRL & 0.696 & 0.361 & 0.383 & 194.01 & 303.89 & 0.625  \\
			ReMVC-MSE & 0.517 & 0.127 & 0.151 & 191.68 & 299.91 & 0.632 \\
			ReMVC (ours) & \textbf{0.762} & \textbf{0.474} & \textbf{0.488} & \textbf{189.92} & \textbf{296.26} & \textbf{0.643} \\ \bottomrule
	\end{tabular}}
	\vspace{-0.6cm}
\end{table}

\section{Response to Reviewer 5}

% \textcolor{blue}{Q9: The experiment results are impressive. However, the introduction focusing on issues from a few papers gives readers some reservation regarding the research impact from the improvements. Can more related work be included (esp. in the introduction section) ? }

% \noindent\textcolor{blue}{Q9: The introduction focusing on issues from a few papers. Can more related work be included. }

% A9: Thanks for your comments. 
\noindent\textcolor{blue}{\textbf{Description of the issues of existing methods.}}
% For research impact, region is a basic concepts in urban environment. A better region representation can serve as an important foundation for many real world applications such as urban planning and transportation prediction. % We will follow your comments and introduce more about research impact. 
%
%
The way we motivate our work in Introduction is to point out the issues of various existing methods, including (Wang and Li 2017; Wang et al. 2018; Yao et al. 2018; Fu et al. 2019; Zhang et al. 2019; Zhang et al. 2020). Specifically, we referred to (Zhang et al. 2020; Wang and Li 2017; Zhang et al. 2019; 2020) when discussing the issues of intra-view feature extraction. We referred to (Fu et al. 2019; Zhang et al. 2019; Zhang et al. 2020) when discussing issues of inter-view embedding fusion. That is, we referred to different subsets of existing studies at different places, thus providing an impression that we are tackling the issues of a limited number of existing methods only. In a newer version, we shall make it clear that (1) many existing methods have been proposed for region representation learning based on POI and/or mobility views with all of their references provided collectively and they suffer from various issues; and (2) how these issues are tackled by the proposed techniques.
\if 0
For more related work and issues, in fact, there are some other papers related to region embedding.
The earliest work often pre-defines some heuristic features, and in some supervised learning models, region embedding is indirectly trained as a byproduct. However, these models are either coarse-grained or task related. We also detail some other unsupervised methods in Related Work section, however, they often require rich auxiliary information from social media platforms which is hard to obtain. 

We will follow your comments and discuss more related works and research impact in our future version.
\fi

